Homotopy Hubbard Trees for post-singularly finite exponential maps

We extend the concept of a Hubbard tree, well established and useful in the theory of polynomial dynamics, to the dynamics of transcendental entire functions. We show that Hubbard trees in the strict traditional sense, as invariant compact trees embedded in $\mathbb{C}$, do not exist even for post-singularly finite exponential maps; the difficulty lies in the existence of asymptotic values. We therefore introduce the concept of a Homotopy Hubbard Tree that takes care of these difficulties. Specifically for the family of exponential maps, we show that every post-singularly finite map has a Homotopy Hubbard tree that is unique up to homotopy, and we show that post-singulary finite exponential maps can be classified in terms of Homotopy Hubbard Trees, using a transcendental analogue of Thurston's topological characterization theorem of rational maps.

==> tikzdefs.tex <==
\tikzset{
  left_axis/.pic={
    % add the left axis with the nodes ks, kinf and (k+1)s
    \node[empty] (base_left) {};
    \node[empty] (top_left) [above=6 of base_left] {};
    \node[empty] (ks)       [above=1 of base_left,label=right:$k\ad{s}$] {};
    \node[empty] (kinf)     [above=1.5 of ks] {};
    \node[empty] (k+s)      [above=4 of ks,label=right:$(k+1)\ad{s}$] {};
    % give each node a tiny horizontal line
    \foreach \n in {ks, kinf, k+s} {
      \draw (\n) ++(-0.1,0) -- ++(0.2,0);
    }
  },
  partition_intervals/.pic={
    % draw the partition sector I and label it
    \node[empty] (I_bottom) [left=2 of ks] {};
    \node[empty] (I_top)    [left=2 of k+s] {};
    \draw[-]     (I_bottom) to node[left,midway]{$I$} (I_top);
    \draw[dotted] (ks) to (I_bottom) to (I_top) to (k+s);
    % draw the partitions I_l and I_u and label them
    \node[empty] (split_bottom)  [left=1 of ks]  {};
    \node[empty] (split_middle)  [left=1 of kinf] {};
    \node[empty] (split_top)     [left=1 of k+s] {};
    \draw[-] (split_bottom) -- node[left,midway]{$I_l$} (split_middle) -- node[left,midway] {$I_u$} (split_top);
    % draw bottom interval markers
    \foreach \n in {I_bottom, split_bottom, split_middle} {
      \node[empty] (c) [above left=0.2 and 0.2 of \n.center] {};
      \draw[] (c.east) arc [start angle=180,end angle=360,radius=0.2];
    }
    % draw top interval markers
    \foreach \n in {I_top,split_middle} {
      \node[empty] (c) [below right=0.2 and 0.2 of \n.center] {};
      \draw (c.west) arc [start angle=0, end angle=180, radius=0.2];
    }
    % the upper bound of I_u includes the boundary
    \draw (split_top.center) ++(-0.2,-0.2) to ++(0,0.2) to ++(0.4, 0) to ++(0, -0.2);
  },
  right_axis/.pic={
    % draw the right axis; give s a tiny horizontal line
    \node[empty] (base_right) [right=2.5 of base_left] {};
    \node[empty] (s)          [above=2.5 of base_right,label=right:$\ad{s}$] {};
    \node[empty] (top_right)  [right=2.5 of top_left] {};
    \draw (s) ++(-0.1,0) -- ++(0.2,0);
  },
  empty/.style={shape=rectangle,inner sep=0},
  interval1/.style={color=red,decoration={snake,amplitude=0.8mm},decorate},
  interval2/.style={color=blue,dashed}
}
